Multimodal Filesystem Memory For Long-Horizon Embodied Agents

Agents operating over long horizons need an effective memory that allows them to reuse their experience throughout long interactions. If the entire history of an interaction is retained, it becomes difficult to find the relevant experience, while compressing it into summaries may result in the loss of visual and spatial details that are required later on. We present \textbf{MFM}, a multimodal filesystem memory architecture that keeps complementary types of agent memory. \textbf{Episodic memory} stores the observations, actions, and outcomes, and \textbf{spatial memory} associates experiences with locations. \textbf{Semantic and procedural memory} build up general knowledge and reusable methods of acting, and \textbf{working memory} holds the current plans. MFM makes use of searchable textual records to connect these different representations to the underlying multimodal episodes. The agents are able to find previous experiences by means of contextual cues and to examine the original observations in order to recover details that are missing from their textual descriptions. Through consolidation, the agents convert experience into higher-level knowledge and procedures while still keeping references to the original episodes. In the case of long-horizon Minecraft and computer-use tasks, MFM leads to improved performance with three base models. With GPT-6-Astra, MFM completes \emph{Mine Diamond from Scratch} and reaches 16 out of 24 milestones on the \emph{Ender Dragon} task, as against 12.7 for the best baseline. On CUABench-KiCad it attains a mean reward of 0.440, as compared to 0.400 for the best baseline and 0.267 in the case of no persistent memory.

==> Sections/app/app_additional_examples_old.tex <==
\section{Additional Examples}
\Cref{fig:tech-tree} shows that MFM enables continued progress toward the Ender Dragon beyond the milestones reached by the baselines. Although VISTA obtains diamond equipment earlier, its progress subsequently plateaus, whereas MFM advances through obsidian and flint and steel to reach netherrack within the same interaction budget.

\begin{figure*}[ht]
  \centering

    \includegraphics[width=\linewidth]{figs/dragon_tech_tree_gpt-6-astra_cap36k_clean.png} 
 



  \caption{\small \textbf{Milestone progression on the Ender Dragon task with gpt-6-Astra.} Curves show progression through the Minecraft technology tree against environment steps (logarithmic scale). Under a shared 36,000-step budget, MFM reaches 16 of 24 milestones, compared with 13 for VISTA, 12 for PRO-LONG, and 6 for direct evaluation (selected single-seed runs). The vertical dashed line marks the interaction budget, and the shaded region indicates milestones no method reached.
  }
  \label{fig:tech-tree}
\end{figure*}






\begin{figure*}[ht]
  \centering
    \includegraphics[width=\linewidth]{figs/steps_per_turn_projected.pdf} 
  \caption{\small \textbf{Environment interaction per agent turn.} Rolling median of environment steps executed per agent turn over each run, across three base models (columns) on Mine Diamond from Scratch (top) and the Ender Dragon (bottom). Higher values indicate more environment interaction between successive agent turns; the vertical axis is logarithmic. Shaded regions mark intervals where MFM exceeds both VISTA and PRO-LONG, with annotations reporting the shaded fraction of each panel.
  }
  \label{fig:steps-per-turn}
\end{figure*}


\begin{figure*}[ht]
  \centering
    \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/kicad/55f2eefb/mfm_gpt6/s009_change_symbol_ok_but_agent_notices_value.png} 
    \caption{\small Task 55f2eefb. }
    \label{fig:s009_change_symbol_ok_but_agent_notices_value}
  \end{subfigure}
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/kicad/c4baee36/mfm_gpt6/s045_finished_schematic_with_48v_and_gnd_symb.png} 
    \caption{\small Task: c4baee36}
    \label{fig:s045_finished_schematic_with_48v_and_gnd_symb}
   \end{subfigure}
      \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/kicad/b7148878/mfm_gpt6/s094_full_schematic.png} 
    \caption{\small Task: b7148878}
    \label{fig:s094_full_schematic}
   \end{subfigure}
   
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/kicad/55f2eefb/vista_gpt56/s010_label_still_reads_9v_on_screen_agent_mis.png} 
    \caption{\small Task: 55f2eefb}
    \label{fig:s010_label_still_reads_9v_on_screen_agent_mis}
  \end{subfigure}
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/kicad/c4baee36/vista_gpt56/s060_local_label_3_3vdc_on_the_output_net.png} 
    \caption{\small Task: c4baee36 }
    \label{fig:s060_local_label_3_3vdc_on_the_output_net}
   \end{subfigure}
   \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/kicad/b7148878/vista_gpt56/s125_saved_done_netlist_r1_1_u2_1_u2_2_dangli.png} 
    \caption{\small Task: b7148878}
    \label{fig:s125_saved_done_netlist_r1_1_u2_1_u2_2_dangli}
   \end{subfigure}
  \caption{\small \textbf{Qualitative comparison on CUABench-KiCad.} Top: results produced by MFM. Bottom: results produced by VISTA on the same three tasks. Columns correspond to Task 55f2eefb, Task c4baee36, and Task b7148878, respectively. }
  \label{fig:kicad-tasks-different-perf}
\end{figure*}


\begin{figure*}[ht]
  \centering
  \begin{subfigure}[t]{0.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/crop_examples/01_frame_640x360_step4588.jpg} 
    \caption{\small Initial observation of a pale animal.}
    \label{fig:crop-wolf-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.34\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/crop_examples/01_zoom_crop.png} 
    \caption{\small Zoomed-in view revealing a wolf.}
    \label{fig:crop-wolf-b}
   \end{subfigure}
   \\
  \begin{subfigure}[t]{0.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/crop_examples/02_frame_640x360_step4917.jpg} 
    \caption{\small Initial observation of a possible pink sheep.}
    \label{fig:crop-sheep-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/crop_examples/02_zoom_crop.png} 
    \caption{\small Zoomed-in view of the sheep.}
    \label{fig:crop-sheep-b}
   \end{subfigure}
  \caption{\small Visual memory inspection for correcting perceptual errors (a–b) and resolving uncertainty (c–d).
  % \textbf{Correcting perceptual errors through visual memory inspection.} al for a sheep. By magnifying the original observation from memory, it correctly identifies the animal as a wolf and revises its plan, avoiding an unnecessary attack.
  % Agent observed a pale animal saw a sheep. By zoomed into the observation from memory, it verified that it is a wolf: do not attack, no fight, no damage. 
   % \textbf{Resolving perceptual uncertainty through visual memory inspection.} The agent is initially uncertain whether the observed animal is a pink sheep. By zooming into the original visual observation, it verifies the sheep and uses this information to guide its subsequent plan for obtaining food and wool.
  % Agent observed but was not sure if it were a pink sheep: food and wool, kill sheep, mutton -> cooked mutton. 
  }
  \label{fig:crop-wolf}
\end{figure*}

\begin{figure*}[ht]
  \centering
  \begin{subfigure}[t]{0.34\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/crop_examples/03_frame_640x360_step884.jpg} 
    \caption{\small Earlier observation of the hole}
    \label{fig:03-a}
  \end{subfigure}
  \begin{subfigure}[t]{0.65\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/crop_examples/03_then_now_sheet.png} 
    \caption{\small Relocating the hole using visual memory}
    \label{fig:03-then-now}
   \end{subfigure}
  \caption{\small \textbf{Memory-guided spatial relocation.} The close visual alignment between the retrieved and current views allows the agent to identify the hole’s rim and recover its precise location.
  }
  \label{fig:03}
  \vskip -0.4cm
\end{figure*}

\begin{figure*}[ht]
  \centering
  \begin{subfigure}[t]{0.34\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/crop_examples/04_frame_640x360_step6138.jpg} 
    \caption{\small Life 1: original observation}
    \label{fig:04_frame_640x360_step6138}
  \end{subfigure}
  \begin{subfigure}[t]{0.65\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/crop_examples/04_then_now_sheet.png} 
    \caption{\small Life 2: retrieved memory vs. current observation}
    \label{fig:04_then_now_sheet}
   \end{subfigure}
  \caption{\small \textbf{Cross-life visual memory retrieval.} Agent retrieves an observation from Life 1 and compares it against its current view in Life 2, correctly recognizing that the live bank is the entrance to Life 1’s iron mine.
  %  1's frame  (a life two generations back)	the live bank is that life's iron entrance	mine iron ore verified at step 6565, first ore of the life
  }
  \label{fig:04}
\end{figure*}

\begin{figure*}[ht]
  \centering
  \begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/crop_examples/05_frame_640x360_step1855.jpg} 
    \caption{\small Retrieved frame with incorrect viewing angle}
    \label{fig:05_frame_640x360_step1855}
  \end{subfigure}
  \begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/crop_examples/05_viewed_frame_ep_000126_step1777.png} 
    \caption{\small Re-aimed view for continued mining}
    \label{fig:05_viewed_frame_ep_000126_step1777}
   \end{subfigure}
  \caption{\small \textbf{Using visual memory to recover mining orientation.} After retrieving the previous entry’s frame, the agent recognizes that the recorded view is aimed upward rather than toward the mining face. It adjusts its view accordingly and resumes mining from the correct orientation.
  % view of the last entry's frame	the aim pointed up, not at the feet	look\_abs re-aim, level floor next turn
  }
  \label{fig:05}
\end{figure*}


Figures \ref{fig:4_erc_practice_ba34f1c3}, \ref{fig:4_erc_practice_4c913e30}, \ref{fig:4_erc_practice_5dbc9e02} show how MFM verifies its own edits on the three CUABench-KiCad tasks discussed in \Cref{sec:qualitative}. In each case, the agent follows the same three-step routine, which it first performed in an earlier task and later retrieved from episodic memory (cf. \Cref{fig:}): it inspects the schematic to confirm that component values and net labels match the specification (a), opens the Electrical Rules Checker (b), and reads the ERC report to confirm that only the expected undriven-power warnings remain and that no pins are left unconnected (c). Checking the resulting application state, rather than trusting the edit operation's "OK" response, allows MFM to catch incomplete edits that VISTA records as successful (\Cref{fig:kicad-tasks-different-perf}).

\begin{figure*}[ht]
  \centering
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/kicad/4_erc_practice/ba34f1c3_step_45.png} 
    \caption{\small The label and all five nets match the design. The title and status bar confirm the schematic is saved.  }
    \label{fig:ba34f1c3_step_45}
  \end{subfigure}
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/kicad/4_erc_practice/ba34f1c3_step_46.png} 
    \caption{\small ERC is open and ready; no feedback errors appear.  }
    \label{fig:ba34f1c3_step_46}
   \end{subfigure}
   \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/kicad/4_erc_practice/ba34f1c3_step_47.png} 
    \caption{\small ERC shows only the two expected undriven-power errors, with zero warnings.  }
    \label{fig:ba34f1c3_step_47}
   \end{subfigure}
  \caption{\small  Task ba34f1c3: open ERC, dialog, results. }
  \label{fig:4_erc_practice_ba34f1c3}
\end{figure*}

\begin{figure*}[ht]
  \centering
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/kicad/4_erc_practice/4c913e30_step_76.png} 
    \caption{\small The wiring matches the committed design, and the schematic is saved in the required directory. }
    \label{fig:4c913e30_step_76}
  \end{subfigure}
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/kicad/4_erc_practice/4c913e30_step_77.png} 
    \caption{\small ERC is ready; no feedback errors appear.  }
    \label{fig:4c913e30_step_77}
   \end{subfigure}
   \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/kicad/4_erc_practice/4c913e30_step_78.png} 
    \caption{\small ERC reports only the three expected undriven-power errors for the external supplies, with zero warnings. The schematic is saved.}
    \label{fig:4c913e30_step_78}
   \end{subfigure}
  \caption{\small Task 4c913e30: opens ERC, dialog, results. }
  \label{fig:4_erc_practice_4c913e30}
\end{figure*}

\begin{figure*}[ht]
  \centering
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/kicad/4_erc_practice/5dbc9e02_step_68.png} 
    \caption{\small The visible values, polarities, and seven nets match the design; no feedback errors appear. }
    \label{fig:5dbc9e02_step_68}
  \end{subfigure}
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/kicad/4_erc_practice/5dbc9e02_step_69.png} 
    \caption{\small The saved title and status bar confirm the schematic’s location. ERC is ready.  }
    \label{fig:5dbc9e02_step_69}
   \end{subfigure}
   \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/kicad/4_erc_practice/5dbc9e02_step_70.png} 
    \caption{\small ERC reports two expected undriven-power errors and zero warnings; no unconnected pins are reported. }
    \label{fig:5dbc9e02_step_70}
   \end{subfigure}
  \caption{\small Task 5dbc9e02: opens ERC, dialog, results. }
  \label{fig:4_erc_practice_5dbc9e02}
\end{figure*}

\begin{figure*}[ht]
  \centering
  \begin{subfigure}[t]{\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/kicad/1_netlist_export_copied/a6414tw4_steps_06-10.png} 
    \caption{\small Current task: \texttt{a6414tw4} }
    \label{fig:a6414tw4_steps_06-10}
   \end{subfigure}

   \begin{subfigure}[t]{\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/kicad/1_netlist_export_copied/4c913e30_steps_78-82.png} 
    \caption{\small Retrieved experience from an earlier task: \texttt{4c913e30}}
    \label{fig:4c913e30_steps_78-82}
  \end{subfigure}


  \caption{\small \textbf{Cross-task reuse of episodic memory in KiCad.} \textbf{Top:} Interaction with the current task (\texttt{a6414tw4}).
\textbf{Bottom:} The agent retrieves an earlier task (\texttt{4c913e30}) with a nearly identical action sequence: save the blank schematic, navigate to \emph{Export} $\rightarrow$ \emph{Netlist}, select the native KiCad format, and specify the output path. 
The retrieved episode provides a concrete precedent for this task. 
}
  \label{fig:kicad-cross-task-reuse}
\end{figure*}


% \subsection{Additional Related Works}

==> Sections/app/app_impl_details_old.tex <==
\section{Harness and Implementation Details}
\label{sec:impl-details}
% \subsection{Harness-provided recall}
% \label{sec:harness-provided-recall}
% Define a repetition streak and the KiCad transition score, including the candidate history used by each heuristic. Keep this scoring distinct from the unranked explicit search above.

 % In Minecraft, this block includes at most two repetition streaks from the last 30 episodes and three earlier episodes within six blocks in the $x$--$z$ plane, excluding the six most recent episodes from the proximity lookup. In KiCad, it contains the three highest-scoring prior transitions, with ties resolved in favor of newer transitions. Each recall line cites the episode identifiers from which it was computed. The agent can inspect these references in the same manner as those returned by explicit search. Automatic recall makes selected history immediately available, while $R_t$ reflects the agent's additional query.

\begin{promptbox}[label={box:index-example}]{Example rows from \texttt{index.jsonl} files.}

\{"action kind": "harvest tree" "first step":0, "last step": 329, "id": "ep 000001" "kind": "episode" "path": "episodes/ep 000001" "summary": " [ACTION]
harvest tree(logs=4,n=400) → 400 ticks: moved 11.8, inv (bucket': 1,
'dirt':
5)", "tags": ["inventory changed", "broke", "note"], "x": 3170.5, "y": 69.0, "z": 1402. 5 \}


\{ "action kind": "go to" "first step":2444, "last step":2452, "id": "ep 000048" "kind": "episode" "summary": "[ACTION] go to(x=3153.4,z=1401.4, within=0.8, n=260) → 260 ticks: moved 0.2", "tags": ["stuck", "note"], "x": 3158.30, "y": 57.0, "z": 1400.53 \}


\{"action kind": "use at" "first step":2318, "last step": 2327, "id": "ep 000043" "summary":" [ACTION]
use at (x=3168, y=64, z=1420, item=water bucket, face=below, hold=1) - 53 ticks: moved 0.0, inv {bucket': 1, 'water bucket': -1}, milestone
['water\_1']", "tags": ["milestone", "inventory\_changed", "note"], "x": 3168.66, "y": 64.0, "z": 1419.47 \}

\end{promptbox}


\textbf{Grids Map.} We have five kinds of "walked", "placed", "opened", "hazard", "blocked". Below, we provide one example for each kind:
\begin{tcolorbox}[
    enhanced,
    colback=gray!3,
    colframe=gray!50,
    boxrule=0.5pt,
    arc=2mm,
    left=3mm,
    right=3mm,
    top=2mm,
    bottom=2mm,
    breakable
]

\{"cell": [-3010, 71, -5573], "kind": "walked", "step": 1\}

\{"cell": [-3017, 49, -5569], "item": "furnace", "kind": "placed", "pose": {"pitch": 55.0, "x": -3017.7, "y": 49.0, "yaw": 270.0, "z": -5568.37}, "step": 4841 \}


\{"cell": [-3009, 69, -5566], "item": "crafting\_table", "kind": "opened", "pose": \{"pitch": 55.0, "x": -3007.43, "y": 69.0, "yaw": 90.0, z: -5565.54\}, "step": 1206 \}

\{"cell": [-3008, 61, -5569], "kind": "blocked", "step": 1961 \}

\{"cell": [-3019, 34, -5569], "damage": 3.0, "kind": "hazard", "step": 6361, "what": "damage"\}


\end{tcolorbox}


Two rows of \Cref{tab:arm-capabilities}: Plan cap and Session policy, may look like they are held constant, because they are intrinsic to each method's published interface. PRO-LONG and MFM are text-first: the model's context is a single running thread of textual records (plans, actions, state blocks, notes), which is cheap to keep resident and can be compacted at 100k tokens without discarding anything the agent could not recover from the log. VISTA, by contrast, is a frame-first harness whose memory is the archive of retained observations, so its context budget is naturally measured in image bytes rather than tokens; once the 4 MB image budget is reached it checkpoints and continues from the archive, and its play/inspect interface issues one plan entry per play because each play returns the frames the model will later revisit. We keep each arm's native policy because forcing VISTA into a token-based compaction schedule (or PRO-LONG into an image budget) would change the method itself rather than equalize the comparison. None of these settings changes what an arm can do in the environment: the 400-step plan horizon, the episode budgets, the 28-atom procedure set, the action reference, and the per-turn state block are identical across arms, so the comparison in \Cref{tab:mcu} and \Cref{tab:kicad} isolates the memory mechanism rather than differences in context packaging.


We did not alter the core algorithms of PRO-LONG or VISTA. Their distinct operational characteristics (e.g., PRO-LONG's text logs and VISTA's visual history buffers) were faithfully ported. The differences in parameters like session policy or plan cap reflect each method's native design requirements (e.g., VISTA relies heavily on recent visual frames, whereas MFM utilizes a multi-stage filter-then-inspect relational index).

% Requires: \usepackage{booktabs,array,tabularx}
% Table 1: per-arm capabilities on the  chassis (gen-4 runs).
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabularx}{\textwidth}{@{}>{\raggedright\arraybackslash}p{3.1cm} >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X@{}}
\toprule
\textbf{Capability} & \textbf{Direct} & \textbf{PRO-LONG} & \textbf{VISTA} & \textbf{MFM} \\
\midrule
Standing brief & full brief (12\,KB), \texttt{AGENTS.md} & full brief (12\,KB), \texttt{AGENTS.md} & full brief (12\,KB), developer instructions & full brief (12\,KB) \\
% Brief read by the model & first 32\,KiB (codex cap) & first 32\,KiB & all & all \\
Procedure set & 28 atoms & 28 atoms & 28 atoms & 28 atoms \\
% Harness guards and governor & on & on & on & off \\
Per-turn \texttt{[RECENT]} / \texttt{[MAP]} & no & yes & yes & yes \\
Episode store and query tool & no & no & archived frames via \texttt{inspect} & yes \\
Write access to own files / procedure execution & yes & yes & yes & yes \\
Agent-written procedures (observed) & 0 & 0 & 0 & 4 written / 14 calls \\
Plan cap & 400 steps & 400 steps &  400 steps &  400 steps \\
Session policy & one turn per call & one thread, compaction at 100k tokens & one thread, 4\,MB image budget, then checkpoint & one thread, compaction at 100k tokens \\
Images per call & current frame & current frame & current frame & current frame + any frame it opens \\
\bottomrule
\end{tabularx}
\caption{Per-arm capabilities on Minecraft tasks. All arms share the action and procedure reference, the knowledge sections, the ground-truth rules, and the per-turn state block. All arms can write files and execute stored procedures through the same interface.
% ; the second row reports how many procedures each arm actually authored across all runs.
% The 32\,KiB cap is the default \texttt{project\_doc\_max\_bytes} of \texttt{codex exec}.
% The MFM arm ran on the minimal contract with the atom procedure set and without the harness safety layer; 
}
\label{tab:arm-capabilities}
\end{table*}


% Requires: \usepackage{booktabs,tabularx}
\begin{table*}[t]\centering\footnotesize\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{\textwidth}{@{}l>{\raggedright\arraybackslash}X@{}}\toprule
\textbf{Atom} & \textbf{What it does} \\ \midrule
\multicolumn{2}{@{}l}{\emph{Aiming and walking}} \\
\texttt{look} & Turn the camera by a relative (pitch, yaw) in degrees, in safe increments. \\
\texttt{look\_at} & Aim the crosshair at a WORLD coordinate (exact, from {[}STATE{]} ground truth). \\
\texttt{look\_abs} & Steer the camera to an ABSOLUTE pitch/yaw, closed-loop against {[}STATE{]} every step (works from any starting pose; `look` is relative). \\
\texttt{go\_to} & Walk to a WORLD (x, z), re-aiming against {[}STATE{]} every step until within reach. \\
\texttt{watch} & Do nothing for up to `n` steps and stop the moment `until` holds, read from the game's own numbers: none (a plain wait), inventory (any count changes), gui (a screen opens), health, damage, y\_below:$<$v$>$, y\_above:$<$v$>$, moved:$<$blocks$>$. \\
\multicolumn{2}{@{}l}{\emph{Mining and pickup}} \\
\texttt{mine\_ahead} & Hold attack on exactly what the crosshair is on -- no re-aiming, no walking. \\
\texttt{collect\_drops} & Walk a small out-and-back sweep to pick up floating item drops; stops the moment the inventory count rises, and says so either way. \\
\multicolumn{2}{@{}l}{\emph{Inventory and GUI cursor}} \\
\texttt{equip\_hotbar} & Select hotbar slot 1-9. \\
\texttt{open\_inventory} & Press E to open the inventory GUI. \\
\texttt{close\_inventory} & Press E to close the screen. \\
\texttt{cursor\_to\_slot} & Land the cursor ON a player inventory slot, by its {[}INV{]} slot id. \\
\texttt{cursor\_to\_cell} & Land the cursor ON a crafting or furnace cell (or the output). \\
\texttt{gui\_click} & Left-click at the cursor (pick up / place a stack). \\
\texttt{gui\_right\_click} & Right-click at the cursor (place one item). \\
\texttt{stow\_items} & Bank the cursor stack and the named craft cells into empty inventory slots (deposits the cursor first, then lifts each cell and banks it), so the screen can close without dropping anything. \\
\texttt{discard\_stack} & Throw a whole inventory stack away (there is no drop key): opens the inventory, lifts the stack in `slot`, force-closes so it lands on the floor, and steps back so you do not pick it up again. \\
\texttt{drop\_and\_pickup} & Throw the stack in `slot` on the floor and walk over it, so the game counts a `pickup` of it. \\
\multicolumn{2}{@{}l}{\emph{Crafting and smelting}} \\
\texttt{craft} & ONE call crafts a recipe from your real inventory: lifts each ingredient, right-clicks one into every cell, puts the remainder back, takes the output `count` times, banks it (tools go to the hotbar) and verifies craft\_item. \\
\texttt{place\_and\_open} & Put your crafting\_table or furnace on the ground one block ahead and open its screen (moves it to the hotbar first if needed, verifies the placement on use\_item and the screen kind). \\
\texttt{furnace\_load} & Load the open furnace: n of item (0 = the whole stack) into the smelt cell and enough fuel into the fuel cell (auto picks coal $>$ charcoal $>$ planks $>$ logs $>$ ssteps). \\
\texttt{furnace\_take} & Take the finished output out of the open furnace and bank it (checks the output cell is not empty first; reports what arrived). \\
\multicolumn{2}{@{}l}{\emph{Placing and using items}} \\
\texttt{place\_at} & Put `item` INTO the block cell (x, y, z) by clicking a face of the block it rests on (default: the block BELOW it, i.e. \\
\texttt{use\_at} & Right-click a face of the block at (x, y, z) with `item` selected: pour a water bucket (item=water\_bucket, the ground block), light with flint\_and\_steel, till with a hoe, plant seeds on farmland, shear a pumpkin, open a door / bed, or `item` omitted = use the block with what you hold (a chest, a door). \\
\texttt{use\_held} & Hold `use` with an item selected: draw a bow (hold$>$=25 then it releases), drink a potion (32), look through a spyglass, raise a shield (hold as long as you want to block). \\
\texttt{fill\_bucket} & Fill an EMPTY bucket at water you can see: holds the bucket and sweeps the crosshair over the ground ahead (pitch 18-60, yaw +-40), tapping use at each aim until a filled bucket appears in the inventory (verified on the inventory; it names water\_bucket / lava\_bucket / milk\_bucket, whatever the sweep met). \\
\texttt{throw} & Throw a snowball / egg / ender pearl / eye of ender: taps use `n` times with the item selected; verified on the count going down. \\
\texttt{eat} & Eat food (the best carried when unnamed); holds use ~40 steps. \\
\texttt{pillar\_up} & Jump and place `n` blocks under your feet (each verified on the measured y): a tower to stand on, a lookout, an escape from a mob. \\
\bottomrule\end{tabularx}
\caption{The 28 atom procedures available (\texttt{procedures.ATOMS}): the closed-loop primitives, the GUI cursor, the one-call craft and the placements. 
% The task-shaped macros of the full set (tree, strip mine, shaft, obsidian, portal, Nether, End) are not provided and are refused with a note.
}
\label{tab:atoms}\end{table*}


% Table 2: resource and usage numbers for the GPT-6 Mine Diamond run that reached 10/10.
\begin{table}[t]
\centering
\small
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{@{}lr@{}}
\toprule
\textbf{Quantity} & \textbf{Value} \\
\midrule
Environment steps & 11,999 \\
Model calls & 130 \\
Episodes stored & 636 \\
Episode directory on disk & 46\,MB \\
Index (\texttt{index.jsonl}) size & 313\,KB \\
Full-resolution frames on disk & 720\,MB \\
Query over the full index & 0.3--0.4\,s \\
\texttt{view\_image} calls & 87 \\
Own procedures written / calls & 4 / 14 \\
% Own reflexes written / fires & 4 / 10 \\
\bottomrule
\end{tabular}
% (\texttt{g4\_mfm\_gpt6\_diamond\_v7})
\caption{Storage, retrieval, and memory-use statistics for the GPT-6 Mine Diamond run that reached 10/10 milestones. 
% Evidence links in agent-written notes are a convention that the harness does not check.
}
\label{tab:mfm-numbers}
\end{table}

\input{Sections/dragon_opus_costs_36k}
